Multi-cell Non-coherent Over-the-Air Computation for Federated Edge Learning

In this paper, we propose a framework where over-the-air computation (OAC) occurs in both uplink (UL) and downlink (DL), sequentially, in a multi-cell environment to address the latency and the scalability issues of federated edge learning (FEEL). To eliminate the channel state information (CSI) at the edge devices (EDs) and edge servers (ESs) and relax the time-synchronization requirement for the OAC, we use a non-coherent computation scheme, i.e., frequency-shift keying (FSK)-based majority vote (MV) (FSK-MV). With the proposed framework, multiple ESs function as the aggregation nodes in the UL and each ES determines the MVs independently. After the ESs broadcast the detected MVs, the EDs determine the sign of the gradient through another OAC in the DL. Hence, inter-cell interference is exploited for the OAC. In this study, we prove the convergence of the non-convex optimization problem for the FEEL with the proposed OAC framework. We also numerically evaluate the efficacy of the proposed method by comparing the test accuracy in both multi-cell and single-cell scenarios for both homogeneous and heterogeneous data distributions.

==> Multi-cell Non-coherent Over-the-Air Computation for Federated Edge Learning/acronyms.tex <==
% Acronyms
\acrodef{signSGD}{sign stochastic gradient descend}
\acrodef{MV}{majority vote}

\acrodef{SNR}{signal-to-noise ratio}
\acrodef{RMSE}{root-mean-square error}
\acrodef{OFDM}{orthogonal frequency division multiplexing}
\acrodef{DFT}{discrete Fourier transform}
\acrodef{PSK}{phase-shift keying}
\acrodef{QAM}{quadrature amplitude modulation}
\acrodef{QPSK}{quadrature phase-shift keying}
\acrodef{PMEPR}{peak-to-mean envelope power ratio}
\acrodef{BER}{bit-error ratio}
\acrodef{SNR}{signal-to-noise ratio}
\acrodef{PSD}{power spectral density}
\acrodef{SE}{spectral efficiency}
\acrodef{CP}{cyclic prefix}
\acrodef{AWGN}{additive white Gaussian noise}
\acrodef{CFR}{channel frequency response}
\acrodef{CIR}{channel impulse response}
\acrodef{MMSE}{minimum mean square error}
\acrodef{LMMSE}{linear minimum mean square error}
\acrodef{BPSK}{binary phase shift keying}
\acrodef{BLER}{block-error rate}
\acrodef{ML}{maximum likelihood}
\acrodef{PHY}{physical layer}
\acrodef{PA}{power amplifier}
\acrodef{IDFT}{inverse DFT}
\acrodef{DoF}{degrees-of-freedom}
\acrodef{IoT}{Internet-of-Things}
\acrodef{FDE}{frequency-domain equalization}
\acrodef{FSK}{frequency-shift keying}
\acrodef{FSK-MV}{\ac{FSK}-based \ac{MV}}
\acrodef{PPM}{pulse-position modulation}
\acrodef{PPM-MV}{\ac{PPM}-based \ac{MV}}
\acrodef{RF}{radio-frequency}
\acrodef{IM}{index modulation}
\acrodef{BS}{base station}
\acrodef{MF}{matched filter}

\acrodef{BAA}{broadband analog aggregation}
\acrodef{OBDA}{one-bit broadband digital aggregation}
\acrodef{FEEL}{federated edge learning}
\acrodef{FL}{federated learning}
\acrodef{ED}{edge device}
\acrodef{ES}{edge server}
\acrodef{UL}{uplink}
\acrodef{DL}{downlink}
\acrodef{OAC}[OAC]{over-the-air computation}
\acrodef{TCI}{truncated-channel inversion}
\acrodef{MV}{majority vote}
\acrodef{CNN}{convolution neural network}
\acrodef{ReLU}{rectified-linear unit}
\acrodef{CSI}{channel state information}
\acrodef{PAPR}{peak-to-average power ratio}
\acrodef{iid}[IID]{independent and identically distributed}
\acrodef{5G}{Fifth Generation}
\acrodef{4G}{Fourth Generation}
\acrodef{NR}{New Radio}
\acrodef{LTE}{Long Term Evolution}
\acrodef{RACH}{random-access channel}
\acrodef{DNN}{deep nueral network}
\acrodef{SGD}{stochastic gradient descend}
\acrodef{SGD}{stochastic gradient descend}
\acrodef{signSGD}{sign stochastic gradient descend}

\acrodef{5G}{Fifth Generation}
\acrodef{4G}{Fourth Generation}
\acrodef{NR}{New Radio}
\acrodef{PRACH}{physical random access channel}
\acrodef{PUCCH}{physical uplink control channel}
\acrodef{OFDMA}{orthogonal frequency division multiple access}




==> Multi-cell Non-coherent Over-the-Air Computation for Federated Edge Learning/otherDefinitions.tex <==
% Some math operators
\let\oldnorm\norm   % <-- Store original \norm as \oldnorm
\let\norm\undefined % <-- "Undefine" \norm
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\newcommand\mydots{\hbox to 1em{.\hss.\hss.}}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% Declarations
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{remark}{\color{black} Remark} 
% \newtheorem{example}{\color{black} Example} 

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{\color{black} Remark} 
\newtheorem{example}{\color{black} Example} 

\DeclareMathOperator{\sign}{sign}

% Extend acronym package with first letter caps
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}



==> Multi-cell Non-coherent Over-the-Air Computation for Federated Edge Learning/variables.tex <==
\def\complexNumbers{\mathbb{C}}
\def\realNumbers{\mathbb{R}}
\def\constante{{\rm e}}
\def\constantj{{\rm j}}
%\def\expectationOperator[#1][#2]{{\mathbb{E}_{#2}}\left[#1\right]}
%\def\identiyVector[#1]{\textbf{\textrm{I}}_{#1}}
%\def\zeroVector[#1]{\textbf{\textrm{0}}_{#1}}
\def\EDreceivedsignal[#1][#2]{r^{#1,{#2}}_{\rm ED}}
\def\ESreceivedsignal[#1][#2]{r^{#1,{#2}}_{\rm ES}}
\def\rmsDelaySpread{T_{\rm rms}}
\def\receivedPowerOfED[#1][#2]{P^{#1,#2}_{\rm ED}}
\def\receivedPowerOfES[#1][#2]{P^{#1,#2}_{\rm ES}}
\def\constantPowerOfED{}
\def\constantPowerOfES{}
\def\numberofconnectedED{\numberOfEdgeDevices_{\rm c}}
\def\numberofconnectedES{\numberOfEdgeServers_{\rm c}}
\def\probability[#1]{\mathbb{P}\left({#1}\right)}
\def\binomialRandomVariable[#1][#2]{B(#1,#2)}
\def\indicatorFunction[#1]{\mathbb{I}\left[{#1}\right]}
\def\indexES{s}
\def\indexED{k}
\def\DLchannel[#1][#2]{h^{#1,{#2}}_{\rm DL}}
\def\ULchannel[#1][#2]{h^{#1,{#2}}_{\rm UL}}
\def\noiseEDplus[#1][#2]{\omega^{#1,{#2}}_{\rm ED}}
\def\noiseESplus[#1][#2]{\omega^{#1,{#2}}_{\rm ES}}
\def\psiforp[#1][#2]{\Delta^{#1,{#2}}_{\rm ED}}
\def\deltaofr[#1][#2]{\Delta^{#1,{#2}}_{\rm ES}}
\def\signofdelta[#1][#2]{\textbf{v}^{#1,{#2}}_{\rm ES}}
\def\signofdeltaElement[#1][#2]{v^{#1,{#2}}_{\rm ES}}
\def\signofpsi[#1][#2]{\textbf{v}^{#1,{#2}}_{\rm ED}}
\def\signofpsiElement[#1][#2]{v^{#1,{#2}}_{\rm ED}}
\def\globalgrad[#1]{\textbf{g}^{(#1)}}
\def\indexofconstantvector[#1]{L_{#1}}
\def\constantvector{\textbf{L}}
\def\errorProboInED{\rm{P_{err}}}
\def\errorProboInES{P^{\rm{corr}}_{\rm{ES}}}
\def\numberOfEDsWithCorrectChoice{Z}
\def\numberOfESsWithCorrectChoice{Y}
\def\indexGradient{i}
%\def\indicatorFunction[#1]{\mathbb{I}\left[{#1}\right]}
\def\expectationOperator[#1][#2]{{\mathbb{E}_{#2}}\left[#1\right]}
\def\probabilityIncorrect[#1]{P^{\rm{err}}_{#1}}
\def\numberOFEDsForOptionOne{K^{+}_{\indexES}}
\def\numberOFEDsForOptionSecond{K^{-}_{\indexES}}
\def\numberOFESsForOptionOne{S^{+}_{\indexED}}
\def\numberOFESsForOptionSecond{S^{-}_{\indexED}}
\def\correctDecision[#1]{p_{\textrm{z},#1}}
%\def\incorrectDecision[#1]{q_{\textrm{z},#1}}
\def\incorrectDecision[#1]{{(1-\correctDecision[\indexGradient])}}
\def\correctDecisionED{p_{\textrm{y},\indexGradient}}
%\def\incorrectDecisionED{q_{\textrm{y},\indexGradient}}
\def\incorrectDecisionED{{(1-\correctDecisionED)}}
\def\indexSubcarrier{m}
\def\indexOFDMSymbol{n}
\def\voteInTime[#1]{n^{#1}}
\def\voteInFrequency[#1]{m^{#1}}
\def\randomSymbolAtSubcarrierED[#1]{s_{\rm ED}^{\indexCommunicationRound,{#1}}}
\def\transmittedSymbolAtSubcarrierED[#1]{t_{\rm ED}^{\indexCommunicationRound,{#1}}}
\def\transmittedSymbolAtSubcarrierES[#1]{t_{\rm ES}^{\indexCommunicationRound,{#1}}}
\def\randomizationSymbolAtSubcarrierED[#1]{s_{\rm ED}^{\indexCommunicationRound,{#1}}}
\def\randomizationSymbolAtSubcarrierES[#1]{s_{\rm ES}^{\indexCommunicationRound,{#1}}}
\def\meanOptionOne{\mu^{+}_{{\rm ED,\indexGradient}}}
\def\meanOptionTwo{\mu^{-}_{{\rm ED,\indexGradient}}}
% \def\meanOptionOne{\lambda^{+}_{\indexGradient}}
% \def\meanOptionTwo{\lambda^{-}_{\indexGradient}}
\def\meanOptionOneES{\mu^{+}_{{\rm ES,\indexGradient}}}
\def\meanOptionTwoES{\mu^{-}_{{\rm ES,\indexGradient}}}
\def\noiseVariance{\sigma_{\rm ES}^2}
\def\noiseVarianced{\sigma_{\rm ED}^2}
\def\batchSize{n_{\rm b}}
\def\varianceBound{{\bm \sigma}}
\def\indexCommunicationRound{t}
\def\communicationRounds{T}
\def\learningRate{\eta}
\def\modelParametersOptimal{{\textbf{w}_{\indexED}^{*}}}
\def\modelparameters{\textbf{w}}
\def\modelParameters{\textbf{w}_{\indexED}}
\def\completeData{\mathcal{G}}
\def\localClasses[#1]{\mathcal{C}_{#1}}
\def\modelParametersAtIterationEle[#1][#2]{w^{(#1)}_{#2}}
\def\datasetBatch[#1]{\mathcal{\tilde{D}}_{#1}}
\def\majorityVote[#1][#2]{\textbf{v}^{#1,{#2}}_{\rm ES}}
\def\GlobalusercentricLF[#1][#2]{F_{#1}(#2)}
\def\localdataset[#1]{\mathcal{G}_{#1}}
\def\mappingFunction{{g}}
\def\localGradientSign[#1][#2]{{\bar{\textbf{g}}}_{#1}^{(#2)}}
\def\localGradientSignElement[#1][#2]{{\bar{g}}_{#1}^{(#2)}}
\def\lossFunction[#1]{{F}_{#1}}
\def\globalGradient[#1]{\hat{\textbf{{g}}}^{(#1)}}
\def\localGradient[#1][#2]{\textbf{g}_{#1}^{(#2)}}
\def\localGradientNoIndex[#1]{{\textbf{g}}_{#1}}
\def\ElementsOfGradient[#1][#2]{{g}_{#1}^{(#2)}}
\def\ElementsOfGradientNoindex[#1]{{g}_{#1}}
\def\localGradientStat[#1][#2]{{\tilde{\textbf{g}}}_{#1}^{(#2)}}
\def\localGradientStatElement[#1][#2]{{\tilde{g}^{(#2)}}_{#1}}
\def\localGradientStatNoIndex[#1]{{\tilde{\textbf{g}}}_{#1}}
\def\localGradientStatNoIndexElement[#1]{{\tilde{g}}_{#1}}
\def\SignofUsercentricElement[#1][#2]{\hat{g}^{(#2)}_{#1}}
\def\symbolEnergy{E_{\rm s}}


% FEEL parameters


\def\numberOfEdgeServers{S}
\def\numberOfEdgeDevices{K}
\def\dataset[#1]{\mathcal{D}_{#1}}
\def\dataSetCardinality{D}

\def\modelParametersAtIteration[#1][#2]{\textbf{w}^{(#1)}_{#2}}
\def\modelParametersInitial{\textbf{w}}
\def\numberOfModelParametersED[#1]{Q_{#1}}
\def\sampleData[#1]{{\textrm{\textbf{x}}}_{#1}}
\def\indexSampleData{{\ell}}
\def\sampleLabel[#1]{{y}_{#1}}
\def\aggregatedGradientSigns[#1]{\textbf{y}^{(#1)}}
\def\aggregatedGradientSignsEle[#1][#2]{{y}^{(#1)}_{#2}}
\def\indexGradient{i}
\def\globalGradientSignEle[#1][#2]{{v}^{(#1)}_{#2}}
\def\globalGradientSign[#1]{\textbf{v}^{(#1)}}
\def\majorityVoteAtIteration[#1]{\textbf{v}^{(#1)}}
\def\majorityVoteInitial{\textbf{v}}

\def\lossFunctionSampleLocal[#1][#2]{f(#1)}
\def\lossFunctionSample[#1]{f(#1)}
\def\lossFunctionLocal[#1][#2]{F_{#1}(#2)}
\def\lossFunctionGlobal[#1][#2]{F_{#1}(#2)}
\def\lossFunctionGlobal[#1]{F(#1)}

\def\neuralNetworkAtED[#1]{\mathcal{N}_{#1}}

\def\updateRule[#1][#2]{U_{#1}(#2)}
\def\numberOfUpdates{E}


% Signal parameters:


\def\symbolVector[#1]{\textbf{\textrm{d}}_{#1}}
\def\symbolVectorEstimate[#1]{\tilde{\textbf{\textrm{{d}}}}_{#1}}
\def\receivedVector[#1]{\textbf{\textrm{r}}_{#1}}
\def\noiseVector[#1]{\textbf{\textrm{n}}_{#1}}
\def\transmittedVector[#1]{\textbf{\textrm{t}}_{#1}}
\def\idftMatrix[#1]{\textbf{\textrm{F}}_{#1}^{\rm H}}
\def\dftMatrix[#1]{\textbf{\textrm{F}}_{#1}}
\def\transformPrecoder[#1]{\textbf{\textrm{T}}_{#1}}
\def\transformDecoder[#1]{\textbf{\textrm{T}}_{#1}^{\rm -1}}
\def\frequencyMapping{\textbf{\textrm{M}}_{\textrm{f}}}
\def\timeMapping{\textbf{\textrm{M}}_{\textrm{t}}}
\def\channelMatrix[#1]{\textbf{\textrm{H}}_{#1}}
\def\oversamplingFactor{O}
\def\samplePeriod{T_{\rm sample}}
\def\symbolSpacing{T_{\rm spacing}}
\def\timeDomainOFDM[#1]{x(#1)}
\def\timeVar{t}
\def\indexTimeSample{n}
\def\numberOfActiveSubcarriers{M}
\def\idftSize{N}
\def\dataSymbols[#1]{d_{#1}}
\def\cpSize{N_{\rm cp}}
\def\SNR{SNR}
\def\symbolDuration{T_{\rm s}}
\def\Ptransmit{P_{\rm tx}}

\def\channelAtSubcarrier[#1]{h_{#1}}
\def\noiseAtSubcarrier[#1]{n_{#1}}
\def\numberOfOFDMSymbols{N}
\def\asymbolFromED[#1]{d_{#1}}
\def\exponentialIntegral[#1]{{\rm Ei}(#1)}
\def\tciFactor[#1]{p_{#1}}
\def\encoder[#1]{\psi_#1}
\def\symbolEnergy{E_{\rm s}}
\def\numberOfVotingOptions{V}
\def\numberOfVotingOptions{V}
\def\indexVotingOption{v}

\def\threshold{t}
\def\pulseDuration{T_{\rm pulse}}
\def\syncError{T_{\rm sync}}
\def\channelSpread{T_{\rm chn}}
\def\delaySpread{T_{\rm rms}}
\def\guardTimeUniform{T_{\rm g}}
\def\numberOfVotesPerDFTsOFDM{M_{\rm vote}}
\def\uniformGap{M_{\rm gap}}
\def\numberOfElementsInAPulse{M_{\rm pulse}}
\def\symbolsActivatedBins{\textbf{p}}
\def\symbolVectorNotation{\textbf{q}}
\def\symbolVectorNotationReceiver{\tilde{\textbf{q}}}
\def\figuresizeA{3.2in}
\def\symbolsChannel{M_{\rm chn}}

% Security
\def\optimumGeometricMean{{\rm \bf z^*}}
\def\variableForGeoemtricMean{{\rm \bf z}}
\def\variableForGeoemtricMeanIteration[#1]{\variableForGeoemtricMean^{#1}}
\def\anotherIterationIndex{m}
\def\weightDistance[#1]{\alpha_{#1}}
\def\medianDistance[#1]{\beta_{#1}}
\def\smoothFactor{v}

% Assumptions
\def\indexArea{a}
\def\referenceDistanceUplink{r_{\rm UL}}
\def\referenceDistanceDownlink{r_{\rm DL}}
\def\distanceED[#1]{r_{#1}}
\def\pathlossExponent{\alpha}
\def\modelParametersEle[#1]{{w}_{#1}}

\def\nonnegativeConstants{\textbf{L}}
\def\nonnegativeConstantsEle[#1]{L_{#1}}
\def\varianceBoundEle[#1]{\sigma_{#1}}
\def\lossFunctionGlobalMinimum{F^*}

\def\globalGradientElementNoIndex[#1]{{g_{#1}}}
\def\globalGradient[#1]{{\textbf{{g}}}^{(#1)}}
\def\globalGradientElement[#1][#2]{{{g}}^{(#1)}_{#2}}

